Automatic Mapping of Unstructured Cyber Threat Intelligence: An Experimental Study

Proactive approaches to security, such as adversary emulation, leverage information about threat actors and their techniques (Cyber Threat Intelligence, CTI). However, most CTI still comes in unstructured forms (i.e., natural language), such as incident reports and leaked documents. To support proactive security efforts, we present an experimental study on the automatic classification of unstructured CTI into attack techniques using machine learning (ML). We contribute with two new datasets for CTI analysis, and we evaluate several ML models, including both traditional and deep learning-based ones. We present several lessons learned about how ML can perform at this task, which classifiers perform best and under which conditions, which are the main causes of classification errors, and the challenges ahead for CTI analysis.

==> tex/bert.tex <==
\section{Leveraging a pre-trained language model for text classification}
\label{sec:Bert}
Considering the promising results obtained from DL models, through the end of our work, we discovered SecureBERT, a BERT-based Language Model (LM) pre-trained on cybersecurity terms, whose preliminary results have been presented in \cite{secBert}. 
BERT is a multi-layer bidirectional Transformer encoder, composed of 12 layers (transformer blocks), 12 attention heads, and 110 million parameters in its "base" version. Generally pre-trained on Masked Language Modeling (MLM) and Next Sentence Prediction (NSP) tasks, SecureBERT presents only a MLM head layer.  
To provide an extensive overview on all modern methodologies engaged today for text classification, we decided to fine-tune the model on our dataset and build a classifier. SecureBERT presents a BERT core followed by a MLM head layer. We extracted the pre-trained BERT core and built a classifier on top of that adding two layer: dropout layer to prevent overfitting, and linear layer for the classification into 188 different categories. 

